Revisiting Challenges for Selective Data Protection of Real Applications

Selective data protection is a promising technique to defend against the data leakage attack. In this paper, we revisit technical challenges that were neglected when applying this protection to real applications. These challenges include the secure input channel, granularity conflict, and sensitivity conflict. We summarize the causes of them and propose corresponding solutions. Then we design and implement a prototype system for selective data protection and evaluate the overhead using the RISC-V Spike simulator. The evaluation demonstrates the efficiency (less than 3% runtime overhead with optimizations) and the security guarantees provided by our system.

==> figures/conchdesign.tex <==
\begin{figure}[t]
	\centering
	\includegraphics[width=\linewidth]{figures/design.pdf}
	\caption{Sensitive data lifetime phases and corresponding Conch design choices}
	\vspace{-5mm}
	\label{fig:design}
\end{figure}

==> figures/design.tex <==
\begin{figure}[t]
	\centering
	\includegraphics[width=\linewidth]{figures/design.pdf}
	\caption{The Overall Design: Using memory tag and encryption to protect sensitive data confidentiality}
	\label{fig:design}
\end{figure}

==> figures/gconflict.tex <==
\begin{figure}[t]
	\centering
	\includegraphics[width=\linewidth]{figures/gconflict.pdf}
	\caption{The conflict between the tag granularity and memory granularity: The dotted frames represent the state of memory word state after the a and b lines of code. \textbf{?} marks the uncertain tag value}
	\label{fig:gconflict}
\end{figure}

==> figures/hardware.tex <==
\begin{figure}[t]
	\centering
	\includegraphics[width=\linewidth]{figures/hardware_new.pdf}
	\caption{The Conch Architecture: The registers and caches are extended and additional devices such as tag propagation supported pipeline, rule and key registers, and tag cache are introduced.}
	\vspace{-2mm}
	\label{fig:hardware}
\end{figure}

==> figures/impl.tex <==
\begin{figure}[t]
	\centering
	\includegraphics[width=\linewidth]{figures/impl.pdf}
	\caption{The implemented simulator}
	\vspace{-10mm}
	\label{fig:impl}
\end{figure}

==> figures/qarmaenc.tex <==
\begin{figure}[t]
	\centering
	\includegraphics[width=0.85\linewidth]{figures/qarmaenc.pdf}
	\caption{QARMA Encryption. Conch utilizes the QARMA and uses address as tweak value to avoid frequency analysis attack.}
	\vspace{-2mm}
	\label{fig:qarma}
\end{figure}

==> figures/simulation.tex <==
\begin{figure}[t]
	\centering
	\includegraphics[width=3.35in]{figures/simulation.pdf}
	\vspace{-12mm}
	\caption{The simulator framework}
	\label{fig:simulation}
\end{figure}

==> tables/config.tex <==
% \begin{table}[t]
%     \centering
%     \caption{\small{Conch Configuration for Evaluation}}
%     \label{tab:config}
%     \resizebox{0.95\linewidth}{!}{%
%     \begin{tabular}{cc}
%         \toprule
%         Processor 
%         & 
%         \text{Spike} \\
%         Compiler  
%         & 
%         \text{gcc v9.2.0}  \\
%         Kernel    
%         & 
%         \text{Linux 5.4.7} \\
%         \hline
%         \end{tabular}%
%     }
% \end{table}
\begin{table}[t]
    \centering
    \caption{The configuration used in evaluation.}
    \label{tab:config}
    \begin{tabular}{ p{0.45\linewidth}p{0.4\linewidth}  }
     \hline
     %\textbf{Processor}  & Spike 1.0.1-dev \\
     %\textbf{Compiler}   & gcc 9.2.0       \\
     %\textbf{Kernel}     & Linux 5.4.7     \\
     %\hline
     \textbf{CPU Frequency} & 5GHz \\
     \textbf{Cache Line Size} & 64B \\
     \textbf{L1 Instruction Cache} & 64KB, 4-way associative \\
     \textbf{L1 Data Cache} & 64KB, 4-way associative \\
     \textbf{Memory} & 4GB, 4 banks, 1.3GHz \\
     \hline
     \textbf{Tag Cache} & 4KB, 8-way associative \\
     \hline
     \end{tabular}
\end{table}

==> tables/gresult.tex <==
% 如何分析 overtaint 情况: 捕获带 tag 的部分写应该可以
% blowfish: 4 bytes erased, 953160 bytes sensitive data;    4-31188 bytes over; 0.14% overhead
% rijndael: 0 bytes erased. 10292076 bytes sensitive data;  0 bytes over; 0 overhead
% zip30:    7 bytes erased. 19161 byte sensitive data;      24 bytes over; 1.04% overhead
% openssl   4.05% over-tainting, 5.12% under-tainting 94 code locations;  2.16% overhead
\begin{table}[t]
    \centering
    \caption{The result of granularity conflict of 4 applications. In the table, we show the percentage of
    sensitive data that has been over-tagged and extra runtime overhead for each application.}
%    \vspace{-2mm}
    \label{tab:gresult}
    \resizebox{.5\textwidth}{!}{
    \begin{tabular}{|c|c|c|c|c|} 
    \hline
     & blowfish & rijndael & zip30 & OpenSSL \\
    \hline
%    \specialrule{0em}{2pt}{2pt}
%    \hline
    % Under-tagging & 0.0004\% & 0\% & 0.037\% & 4.05\% \\ 
    Over-tagging & 0.033\%/0.14\% & 0\%/0\% & 0.13\%/1.04\% & 5.12\%/2.16\% \\
    \hline
    % \specialrule{0em}{2pt}{2pt}
    % \hline
%    Under-tagging & 0.0004\% & 0\% & 0.037\% & 4.05\% \\ 
    % \hline
    % Extra overhead & 0.14\% & 0\% & 1.04\% & 2.16\% \\
%    \hline
    \end{tabular}
    }
\end{table}


